Position: Solve Layerwise Linear Models First to Understand Neural Dynamical Phenomena (Neural Collapse, Emergence, Lazy/Rich Regime, and Grokking)

In physics, complex systems are often simplified into minimal, solvable models that retain only the core principles. In machine learning, layerwise linear models (e.g., linear neural networks) act as simplified representations of neural network dynamics. These models follow the dynamical feedback principle, which describes how layers mutually govern and amplify each other's evolution. This principle extends beyond the simplified models, successfully explaining a wide range of dynamical phenomena in deep neural networks, including neural collapse, emergence, lazy and rich regimes, and grokking. In this position paper, we call for the use of layerwise linear models retaining the core principles of neural dynamical phenomena to accelerate the science of deep learning.

==> app_empirical.tex <==
\section{Empirical results}\label{app:empirical}



==> app_lin_layerwise_comp.tex <==
\section{Comparison between the inductive bias of linear and layerwise linear models}\label{app:lin_mullin_compare}



The dynamics equation of a linear model with feature map $\Phi$ on trained with GF (\cref{eq:GF}) under MSE loss (\cref{eq:mse}) is
\begin{align}\label{eq:linear_differential}
\frac{df}{dt} = - \eta \mathcal{T}\left[f - f^*\right],
\end{align}
where the integral operator $\mathcal{T}: \mathcal{H} \rightarrow \mathcal{H}$ is
\begin{equation}
    \mathcal{T}[f](x') := \int_\rchi \Phi(x)^T\Phi(x')f(x)q(x)dx.
\end{equation}
The derivation of \cref{eq:linear_differential} follows by expanding $f$ in the features and plugging in \cref{eq:GF} for all parameters
\begin{align}
\frac{df}{dt}(x') &= \sum_k^p \frac{dw_k}{dt}\Phi_i(x') = \sum_k^p  -\eta \frac{d\mathcal{L}}{dw_k}\Phi_k(x') \\
&= - \eta \int_\rchi \left(f(x) - f^*(x)\right) \sum_k^p\frac{df}{dw_k}(x)  q(x) dx \Phi_k(x')\\
&= - \eta \int_\rchi \left(f(x) - f^*(x)\right) \sum_k^p\Phi_k(x) \Phi_k(x') q(x) dx \\
&= - \eta \mathcal{T}\left[f - f^*\right],
\end{align}
where in the second line, we used \cref{eq:mse} and \cref{eq:GF}, and assumed infinite datapoints so $\mathcal{L}_{emp}=\mathcal{L}$. In the last line, we used the definition of integral operator (\cref{eq:operator}). 

Using the eigenvalues $\rho_k$ and eigenfunctions $e_k$ the Hilbert-Schmidt operator $\mathcal{T}$, we obtain the dynamics for each $\braket{e_k|f}$ by inner producting $e_k$ on both sides of \cref{eq:linear_differential},
\begin{align}\label{eq:e_k_dynamics}
\frac{d\braket{e_k|f}}{dt} = \int_\rchi e_k(x')\frac{df}{dt}(x')q(x')dx' &= -\eta \int_\rchi e_k(x')\mathcal{T}\left[f - f^*\right](x') q(x')dx'\\
&= -\eta \braket{e_k|\mathcal{T}| f-f^*} \\
&= -\eta \rho_k (\braket{e_k|f} - \braket{e_k|f^*}).
\end{align}
Expanding $f$ in the eigenfunction basis and plugging in \cref{eq:e_k_dynamics}, the function $f$ at time $t$ is a sum of $p$ independent modes that saturate faster for larger eigenvalues: 
%We obtain the function dynamics by assuming $f$ is a zero function at initialization and expanding $f$ in the eigenfunction basis,
\begin{equation}\label{eq:e_k_dynamics2}
f(x,t) = \sum_{k=1}^p \braket{e_k|f^*} (1-e^{-\eta \rho_k t}) e_k(x),
\end{equation}
where we assumed $f$ is a zero function at initialization. \cref{eq:e_k_dynamics2} shows that GF decouples the dynamics of linear models into $p$ modes, where each mode corresponds to the evolution of $\braket{e_k|f}$ having a saturation speed governed by $\rho_k$.

==> dump.tex <==

A toy scenario with $C=1$, $\eta=1$, and without bias provides a simpler interpretation. The equation of dynamics become
\begin{equation}\label{eq:UFMdynamics}
\frac{dH}{dt} = -(Hw - y)w^T, \quad \frac{dw}{dt} = - H^T(Hw - y).
\end{equation}
where we changed $Y$ to $y$ and $W$ to $w$ to denote that they are column vectors.
Using the two equations above, we can deduce that 
\begin{equation}\label{eq:conservedUFM}
H^T\frac{dH}{dt} - \frac{dw}{dt}w^T = 0,
\end{equation}
or $H^TH - ww^T$ is conserved in the dynamics. Assuming $H^TH - ww^T \approx 0$ for sufficiently small initialization, $H$ is approximately a rank $1$ matrix because it has the same rank as $w \in \mathbb{R}^{p \times 1}$. After training when $H^Tw = y$, the rank $1$ condition and \cref{eq:conservedUFM} results in
\begin{equation}
H = yw^T/\sqrt{\|w\|}, \quad\quad \|w\|^2 = \|y\|,
\end{equation}
impling the feature matrix has \textbf{one} feature parallel to $w$ and the weight matrix (vector) $w$ projects $H$ along $w$ to reproduce $y$. 

See the papers for the derivation.




In the unconstrained feature model, the first matrix $H$ describes the unconstrained features (



to describe the NC. UFM, similar to matrix factorization \cite{gunasekar2017implicitregularizationmatrixfactorization}, consists of a feature matrix $H \in \mathbb{R}^{n \times p}$ representing the last layer features, a last layer weight matrix $W \in \mathbb{R}^{p \times C}$, and a bias vector $b \in \mathbb{R}^{p}$  (\cref{fig:unconstrained_setup}). The entire model, including the feature matrix $H$, is trained on GF to fit the labels $Y \in \mathbb{R}^{n \times C}$. Because we train the feature matrix without any constraints from inputs or transformations, the model is called the `unconstrained feature' model.





\paragraph{Dynamics} We can also show that $H$ collapse into a rank 1 matrix from the dynamics. Specifically, the norm of $H$ along the compliment of $y$ decays when $\| H^TH-ww^T \| \ll 1$. For $P = I - yy^T/\|y\|$, the projection matrix on the compliment of $y$, the dynamics of $PH$ is 
\begin{equation}
P\frac{dH}{dt} = -PH(H^TH - \epsilon),
\end{equation}
where we replace $ww^T$ with a small matrix $\epsilon=H^TH-ww^T$ and $H^TH$. The dynamics of the norm is
\begin{align}
\frac{d}{dt}Tr(PHH^TP) &= Tr(P \frac{dH}{dt} H^TP) + Tr(P H\frac{dH^T}{dt} P) \\
&= -2Tr(PHH^THH^TP) + 2Tr(PH\epsilon H^TP).
\end{align}
Because $Tr(PHH^THH^TP)$ is always a positive constant, taking $\epsilon \rightarrow 0$ assures that the norm of $PH$ decays over time. This shows that the left eigenspace of $H$ reduces to a 1-dim space parallel to $y$, making $H$ a rank-one matrix.


Generalizing the argument to $C > 1$ and plugging in 
\begin{equation} \label{eq:labelmatrix_shape}
Y^T = \begin{pmatrix} 
\boxed{\begin{matrix} 1 & \cdots & 1 \end{matrix}} & & & 0 \\
 & \boxed{\begin{matrix} 1 & \cdots & 1 \end{matrix}} & & \\
& & \ddots & \\ 
0 & & & \boxed{\begin{matrix} 1 & \cdots & 1 \end{matrix}}
\end{pmatrix}.
\end{equation}
leads to the NC conditions with $C$ features. See reference for more rigorous proofs \cite{mixon2020neural,fang2021layer,han2021neural}.
\cite{mixon2020neural,fang2021layer} used the dynamics of UFM (a two layer linear neural network) to show the Neural Collapse.


For demonstrative purposes, asssume a 2-layer neural network with a nonlinearity. The update of the first layer will alter the features and thus change the kernel while the update of the last will lead to only a linear solution. Making a careful initialization and normalization scheme so the update of the last layer is more dominant and the solution is achieved before the significant update of the first layer is the key.

\paragraph{Scaling argument for NTK} For example in the NTK, let $d_2$
\begin{equation}
f(x) = \frac{1}{\sqrt{d_2}}\sigma(xW)w, \quad W \in \mathbb{R}^{d_1 \times d_2}, w \in \mathbb{R}^{d_2},
\end{equation}
where $\sigma$ is the nonlinearity. Let us assume $W \sim \mathcal{N}(0,\alpha^2I)$ and $w \sim \mathcal{N}(0,\beta^2)$. The goal is to fit the data (assumes $\mathcal{O}(1)$ scale) with negligible update in $W$.  

We are happy to update the last layer and we want to achieve after training that $\mathcal{f(x)} = \frac{1}{\sqrt{d_2}} d_2 \alpha \beta \approx 1$ while $dW/dt / dw/dt \ll 1$ or $a \ll \beta$.

Loosely speaking, if the features of 
See the scaling argument in \cite{luo2021phase} for more thorough explanation, and related works \cite{kunin2024get, domine2024lazy} for more specific crtieria. 

Because the last layer is a linear layer, updating the last layer does not alter the NTK. The key for fixing the NTK is to update mostly the last layer while keeping the update of the earlier layers small enough that they don't change much.


 
 [get rich quick]


 \paragraph{Model}
For simplicity, we will assume the following $x_{ki}x_{kj} = 0$ for $i \neq j$ to simplify the math, and assume the input features have unit variance and zero mean. 

We will assume a finite datapoints.


\paragraph{Lazy regime with infinitesimal target scale.}
Now we will assume the initialization scale of [SMTH], then the equation shows that small change in feature can lead to large increase in the loss due to the coupling term.


We won't go too far in to the lazy regime, instead, we will look on the other end, where the extreme rich regime.
Based on this idea, we present another layerwise linear model that 

Chizat uses centered initalization or symmetriczed initalization which sticks the feature in place! b

The layerwise linear models can also explain this in terms of initialization.

\paragraph{Intuition} The larger weights can be understood as heavy weights that does not change much during training. The conserve quantity keeps the difference of the norm fixed, meaning the sufficient difference in initialization leads to the only a neglegible change only for hte 


easier to understand from this perspective. 


The weakly coupled multilinear model is simpler than the linear neural network because each hidden node maps to a feature instead of a linear combination of the hidden nodes. The dynamics of the coupled multilinear model is
\begin{align}\label{eq:coupled1}
\frac{da_{ki}}{dt} = -\eta b_k \sum_{\alpha=1}^n\sum_{\beta=1}^n\left(b_ka_{ki} + \sum_{j \neq i} b_k a_{kj} x_{ki}^{(\alpha)}x_{kj}^{(\beta)}) + \sum_{l \neq k} \sum_{j} b_{lj} a_{lj} x_{ki}^{(\alpha)} x_{lj}^{(\beta)} - x_{ki}^{(\alpha)}y^{(\beta)} \right),
\end{align}
and
\begin{align}\label{eq:coupled2}
\frac{db_{k}}{dt} = -\eta \sum_{\alpha=1}^n\sum_{\beta=1}^n\left( \sum_i a_{ki} x_{ki}^{(\alpha)}  \right) \left(b_k a_{kj}x_{kj}^{(\beta)} + \sum_{l\neq k}\sum_{j} b_l a_{lj} x_{lj}^{(\beta)} - y^{(\beta)} \right).
\end{align}
Note the additional coupling term (\cref{fig:divided_terms}) that is absent in \cref{eq:decoupled_dynamics2}. The coupling term will vanish for infinite training points $n \rightarrow \infty$, but plays a role in the dynamics for finite datapoints.

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.99 \columnwidth]{figures/divided_terms2.drawio.pdf}
\end{center}
\caption{\textbf{Term labels} The term labels of \cref{eq:coupled2}. Because the $k^{\mathrm{th}}$ feature is $\sum_i a_{ki} x_{ki}$, the self-intensity term measures the norm of the feature and the coupling term the inner product between features over the training set.}\label{fig:divided_terms}
\end{figure}


\paragraph{Decoupled scenario} When the coupling terms are negligible, for example when $a_{ki}, b_k \ll 1$ for all $k$ and $i$, the coupled multilinear model simplifies to the extended multilinear model studied in \cref{ch:3-emergence}, or the small initialization scenario in linear neural networks or UFM. Analogous to the proof of \cref{lemma2}, the gradient for $a_{ki}$ flows in a direction parallel to $[\sum_{\alpha}^n x_{k1}^{(\alpha)} y^{(\alpha)}, \cdots, \sum_{\alpha}^n x_{kd}^{(\alpha)} y^{(\alpha)}]$, aligning the features such that $[\sum_{i} a_{ki}x_{ki}^{(1)}, \cdots, \sum_{i} a_{ki}x_{ki}^{(n)}] \propto  [y^{(1)}, \cdots, y^{(n)}]$ for all $n$ training points. 

After the initial alignment, the features increase their intensity by \cref{eq:saxe_analytic}. Assuming the initialization is small enough, the most aligned feature -- or the feature that aligns the target the fastest -- with the largest correlation $\lambda_i = \sum_{i} \sum_{\alpha}^n a_{ki}x_{ki}^{(\alpha)} y^{(\alpha)}$ emerges and saturates before any other features, thus the MF regime (\cref{fig:coupling_fig}(a)).  

%in which case, the most useful feature, typically the most  and the dynamics \cref{eq:coupled1,eq:coupled2} reduces to the scaling of the feature (\cref{eq:decoupled_dynamics2}), reaching the MF regime.

\paragraph{Strongly coupled scenario} If the coupled term dominates the dynamics, the gradients will prioritize orthogonalizing the features rather than fitting the training targets. If multiple features have significant intensities, orthogonalizing features result in the gradients flowing in multiple directions and suppress the alignment of one (as the target function is a scalar output function) feature from dominating the dynamics: suggesting an EF regime (\cref{fig:coupling_fig}(b)). 

\section{Inductive bias for salient features}
In \cref{eq:dynamics_linear}, linear models are biased toward larger features (with larger $\mathbf{E}[x_i^2]$), saturating them first. In contrast, the diagonal linear neural network (\cref{eq:dynamics}) saturates the most salient feature, defined by the largest input-output correlation $S_i\mathbf{E}[x_i^2] = \mathbf{E}[xf^*(x)]$, as shown in the saturation time scale:
\begin{align}
\tau^{(lin)} &\sim 1/\mathbf{E}[x_i^2], \quad \tau^{(diag)} \sim 1/(S_i\mathbf{E}[x_i^2]).
\end{align}
The inductive bias of diagonal linear neural network suggests that it will learn the most relevant features first, suggesting how the model can be more task-adaptive.\footnote{We refer to the dynamical inductive bias of model, and do not consider inductive bias in terms of generalization.} In this section, we present how the dynamics toward salient features and the stage-like training can explain Neural Collapse.

\begin{figure}[h]
\centering
\subfloat[Decoupled scenario: smaller initialization, smaller input scale, larger target scale]{
\includegraphics[width=\columnwidth]{figures/grokless_all.pdf}}
\hfill
\subfloat[Coupled scenario: larger initialization, larger input scale, smaller target scale]{
\includegraphics[width=\columnwidth]{figures/grok_all.pdf}
}
\caption{\textbf{Decoupled/coupled dynamics of the coupled multilinear model} The feature quality, feature norm, and train/test accuracies are plotted against steps for both decoupled (a) and coupled (b) setups, with each color representing one of the 8 features. \textbf{(i):} The test (solid) and train (dashed) quality (\cref{eq:train_test_qual}) indicate how well the features represent the target function and training labels, respectively. For the decoupled case, the first feature (blue) has significantly higher training quality at step $10^2$ but is on par with other features for the coupled case.
\textbf{(ii):} The feature norm (\cref{eq:norm_couple}) measures a feature's size relative to the target function's norm. In the decoupled case, the first feature solely dominates, while in the coupled case, all feature norms exceed the target function's norm at initialization, with the first feature's dominance delayed until after significant weight decay. \textbf{(iii):} The training (dashed) and test (solid) accuracy. The decoupled case shows agreement between accuracies, while the coupled case results in grokking.}\label{fig:grokking_all}
\end{figure}

\subsection{Application: grokking}
Grokking or delayed generalization refers to the sudden catch-up of the test error after signifant amount of time has passed with high training accuracy. As studied in [REF], grokking is a transition from the lazy to rich regime. We empirically demonstrate that properties that respect features leads to grokking dynamics instead of the greedy dynamics.

The conditions for grokking is that there are insufficient data, sufficient number of "similarly useful" features, initially non-greedy dynamics, and finally a method (e.g. a regulation) to promote greedy dynamics. 

We define the prudent dynamics, dynamics where many features are updated at similar scale, in contrast to the greedy dynamics. In this regime may be non-linear, but feature learning is less strong. In other words, instead of feature-learning a few "relevant" features, we will be using many "less suitable" features. 


In the general dynamics of linear neural networks, we have the entangled term that we ignored thanks to small initialization. Englarging this terms creates more coupling [WHY?], while reducing it leads to more decoupled greedy dynamics. Note that techniques for reducing this term -- reducing input std, reducing initialization, increasing target size, more datapoints, and dropouts for decoupling -- leads to instant generalizing dynamics instead of delayed generalization.


\section{Electronic Submission}
\label{submission}

Submission to ICML 2024 will be entirely electronic, via a web site
(not email). Information about the submission process and \LaTeX\ templates
are available on the conference web site at:
\begin{center}
\textbf{\texttt{http://icml.cc/}}
\end{center}

The guidelines below will be enforced for initial submissions and
camera-ready copies. Here is a brief summary:
\begin{itemize}
\item Submissions must be in PDF\@. 
\item \textbf{New to this year}: If your paper has appendices, submit the appendix together with the main body and the references \textbf{as a single file}. Reviewers will not look for appendices as a separate PDF file. So if you submit such an extra file, reviewers will very likely miss it.
\item Page limit: The main body of the paper has to be fitted to 8 pages, excluding references and appendices; the space for the latter two is not limited. For the final version of the paper, authors can add one extra page to the main body.
\item \textbf{Do not include author information or acknowledgements} in your
    initial submission.
\item Your paper should be in \textbf{10 point Times font}.
\item Make sure your PDF file only uses Type-1 fonts.
\item Place figure captions \emph{under} the figure (and omit titles from inside
    the graphic file itself). Place table captions \emph{over} the table.
\item References must include page numbers whenever possible and be as complete
    as possible. Place multiple citations in chronological order.
\item Do not alter the style template; in particular, do not compress the paper
    format by reducing the vertical spaces.
\item Keep your abstract brief and self-contained, one paragraph and roughly
    4--6 sentences. Gross violations will require correction at the
    camera-ready phase. The title should have content words capitalized.
\end{itemize}

\subsection{Submitting Papers}

\textbf{Paper Deadline:} The deadline for paper submission that is
advertised on the conference website is strict. If your full,
anonymized, submission does not reach us on time, it will not be
considered for publication. 

\textbf{Anonymous Submission:} ICML uses double-blind review: no identifying
author information may appear on the title page or in the paper
itself. \cref{author info} gives further details.

\textbf{Simultaneous Submission:} ICML will not accept any paper which,
at the time of submission, is under review for another conference or
has already been published. This policy also applies to papers that
overlap substantially in technical content with conference papers
under review or previously published. ICML submissions must not be
submitted to other conferences and journals during ICML's review
period.
%Authors may submit to ICML substantially different versions of journal papers
%that are currently under review by the journal, but not yet accepted
%at the time of submission.
Informal publications, such as technical
reports or papers in workshop proceedings which do not appear in
print, do not fall under these restrictions.

\medskip

Authors must provide their manuscripts in \textbf{PDF} format.
Furthermore, please make sure that files contain only embedded Type-1 fonts
(e.g.,~using the program \texttt{pdffonts} in linux or using
File/DocumentProperties/Fonts in Acrobat). Other fonts (like Type-3)
might come from graphics files imported into the document.

Authors using \textbf{Word} must convert their document to PDF\@. Most
of the latest versions of Word have the facility to do this
automatically. Submissions will not be accepted in Word format or any
format other than PDF\@. Really. We're not joking. Don't send Word.

Those who use \textbf{\LaTeX} should avoid including Type-3 fonts.
Those using \texttt{latex} and \texttt{dvips} may need the following
two commands:

{\footnotesize
\begin{verbatim}
dvips -Ppdf -tletter -G0 -o paper.ps paper.dvi
ps2pdf paper.ps
\end{verbatim}}
It is a zero following the ``-G'', which tells dvips to use
the config.pdf file. Newer \TeX\ distributions don't always need this
option.

Using \texttt{pdflatex} rather than \texttt{latex}, often gives better
results. This program avoids the Type-3 font problem, and supports more
advanced features in the \texttt{microtype} package.

\textbf{Graphics files} should be a reasonable size, and included from
an appropriate format. Use vector formats (.eps/.pdf) for plots,
lossless bitmap formats (.png) for raster graphics with sharp lines, and
jpeg for photo-like images.

The style file uses the \texttt{hyperref} package to make clickable
links in documents. If this causes problems for you, add
\texttt{nohyperref} as one of the options to the \texttt{icml2024}
usepackage statement.


\subsection{Submitting Final Camera-Ready Copy}

The final versions of papers accepted for publication should follow the
same format and naming convention as initial submissions, except that
author information (names and affiliations) should be given. See
\cref{final author} for formatting instructions.

The footnote, ``Preliminary work. Under review by the International
Conference on Machine Learning (ICML). Do not distribute.'' must be
modified to ``\textit{Proceedings of the
$\mathit{41}^{st}$ International Conference on Machine Learning},
Vienna, Austria, PMLR 235, 2024.
Copyright 2024 by the author(s).''

For those using the \textbf{\LaTeX} style file, this change (and others) is
handled automatically by simply changing
$\mathtt{\backslash usepackage\{icml2024\}}$ to
$$\mathtt{\backslash usepackage[accepted]\{icml2024\}}$$
Authors using \textbf{Word} must edit the
footnote on the first page of the document themselves.

Camera-ready copies should have the title of the paper as running head
on each page except the first one. The running title consists of a
single line centered above a horizontal rule which is $1$~point thick.
The running head should be centered, bold and in $9$~point type. The
rule should be $10$~points above the main text. For those using the
\textbf{\LaTeX} style file, the original title is automatically set as running
head using the \texttt{fancyhdr} package which is included in the ICML
2024 style file package. In case that the original title exceeds the
size restrictions, a shorter form can be supplied by using

\verb|\icmltitlerunning{...}|

just before $\mathtt{\backslash begin\{document\}}$.
Authors using \textbf{Word} must edit the header of the document themselves.

\section{Format of the Paper}

All submissions must follow the specified format.

\subsection{Dimensions}




The text of the paper should be formatted in two columns, with an
overall width of 6.75~inches, height of 9.0~inches, and 0.25~inches
between the columns. The left margin should be 0.75~inches and the top
margin 1.0~inch (2.54~cm). The right and bottom margins will depend on
whether you print on US letter or A4 paper, but all final versions
must be produced for US letter size.
Do not write anything on the margins.

The paper body should be set in 10~point type with a vertical spacing
of 11~points. Please use Times typeface throughout the text.

\subsection{Title}

The paper title should be set in 14~point bold type and centered
between two horizontal rules that are 1~point thick, with 1.0~inch
between the top rule and the top edge of the page. Capitalize the
first letter of content words and put the rest of the title in lower
case.

\subsection{Author Information for Submission}
\label{author info}

ICML uses double-blind review, so author information must not appear. If
you are using \LaTeX\/ and the \texttt{icml2024.sty} file, use
\verb+\icmlauthor{...}+ to specify authors and \verb+\icmlaffiliation{...}+ to specify affiliations. (Read the TeX code used to produce this document for an example usage.) The author information
will not be printed unless \texttt{accepted} is passed as an argument to the
style file.
Submissions that include the author information will not
be reviewed.

\subsubsection{Self-Citations}

If you are citing published papers for which you are an author, refer
to yourself in the third person. In particular, do not use phrases
that reveal your identity (e.g., ``in previous work \cite{langley00}, we
have shown \ldots'').

Do not anonymize citations in the reference section. The only exception are manuscripts that are
not yet published (e.g., under submission). If you choose to refer to
such unpublished manuscripts \cite{anonymous}, anonymized copies have
to be submitted
as Supplementary Material via OpenReview\@. However, keep in mind that an ICML
paper should be self contained and should contain sufficient detail
for the reviewers to evaluate the work. In particular, reviewers are
not required to look at the Supplementary Material when writing their
review (they are not required to look at more than the first $8$ pages of the submitted document).

\subsubsection{Camera-Ready Author Information}
\label{final author}

If a paper is accepted, a final camera-ready copy must be prepared.
%
For camera-ready papers, author information should start 0.3~inches below the
bottom rule surrounding the title. The authors' names should appear in 10~point
bold type, in a row, separated by white space, and centered. Author names should
not be broken across lines. Unbolded superscripted numbers, starting 1, should
be used to refer to affiliations.

Affiliations should be numbered in the order of appearance. A single footnote
block of text should be used to list all the affiliations. (Academic
affiliations should list Department, University, City, State/Region, Country.
Similarly for industrial affiliations.)

Each distinct affiliations should be listed once. If an author has multiple
affiliations, multiple superscripts should be placed after the name, separated
by thin spaces. If the authors would like to highlight equal contribution by
multiple first authors, those authors should have an asterisk placed after their
name in superscript, and the term ``\textsuperscript{*}Equal contribution"
should be placed in the footnote block ahead of the list of affiliations. A
list of corresponding authors and their emails (in the format Full Name
\textless{}email@domain.com\textgreater{}) can follow the list of affiliations.
Ideally only one or two names should be listed.

A sample file with author names is included in the ICML2024 style file
package. Turn on the \texttt{[accepted]} option to the stylefile to
see the names rendered. All of the guidelines above are implemented
by the \LaTeX\ style file.

\subsection{Abstract}

The paper abstract should begin in the left column, 0.4~inches below the final
address. The heading `Abstract' should be centered, bold, and in 11~point type.
The abstract body should use 10~point type, with a vertical spacing of
11~points, and should be indented 0.25~inches more than normal on left-hand and
right-hand margins. Insert 0.4~inches of blank space after the body. Keep your
abstract brief and self-contained, limiting it to one paragraph and roughly 4--6
sentences. Gross violations will require correction at the camera-ready phase.

\subsection{Partitioning the Text}

You should organize your paper into sections and paragraphs to help
readers place a structure on the material and understand its
contributions.

\subsubsection{Sections and Subsections}

Section headings should be numbered, flush left, and set in 11~pt bold
type with the content words capitalized. Leave 0.25~inches of space
before the heading and 0.15~inches after the heading.

Similarly, subsection headings should be numbered, flush left, and set
in 10~pt bold type with the content words capitalized. Leave
0.2~inches of space before the heading and 0.13~inches afterward.

Finally, subsubsection headings should be numbered, flush left, and
set in 10~pt small caps with the content words capitalized. Leave
0.18~inches of space before the heading and 0.1~inches after the
heading.

Please use no more than three levels of headings.

\subsubsection{Paragraphs and Footnotes}

Within each section or subsection, you should further partition the
paper into paragraphs. Do not indent the first line of a given
paragraph, but insert a blank line between succeeding ones.

You can use footnotes\footnote{Footnotes
should be complete sentences.} to provide readers with additional
information about a topic without interrupting the flow of the paper.
Indicate footnotes with a number in the text where the point is most
relevant. Place the footnote in 9~point type at the bottom of the
column in which it appears. Precede the first footnote in a column
with a horizontal rule of 0.8~inches.\footnote{Multiple footnotes can
appear in each column, in the same order as they appear in the text,
but spread them across columns and pages if possible.}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Figures}

You may want to include figures in the paper to illustrate
your approach and results. Such artwork should be centered,
legible, and separated from the text. Lines should be dark and at
least 0.5~points thick for purposes of reproduction, and text should
not appear on a gray background.

Label all distinct components of each figure. If the figure takes the
form of a graph, then give a name for each axis and include a legend
that briefly describes each curve. Do not include a title inside the
figure; instead, the caption should serve this function.

Number figures sequentially, placing the figure number and caption
\emph{after} the graphics, with at least 0.1~inches of space before
the caption and 0.1~inches after it, as in
\cref{icml-historical}. The figure caption should be set in
9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or
bottom of a column, and you may set wide figures across both columns
(use the environment \texttt{figure*} in \LaTeX). Always place
two-column figures at the top or bottom of the page.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
\cref{alg:example} shows an example.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
\cref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.

\subsection{Theorems and such}
The preferred way is to number definitions, propositions, lemmas, etc. consecutively, within sections, as shown below.
\begin{definition}
\label{def:inj}
A function $f:X \to Y$ is injective if for any $x,y\in X$ different, $f(x)\ne f(y)$.
\end{definition}
Using \cref{def:inj} we immediate get the following result:
\begin{proposition}
If $f$ is injective mapping a set $X$ to another set $Y$, 
the cardinality of $Y$ is at least as large as that of $X$
\end{proposition}
\begin{proof} 
Left as an exercise to the reader. 
\end{proof}
\cref{lem:usefullemma} stated next will prove to be useful.
\begin{lemma}
\label{lem:usefullemma}
For any $f:X \to Y$ and $g:Y\to Z$ injective functions, $f \circ g$ is injective.
\end{lemma}
\begin{theorem}
\label{thm:bigtheorem}
If $f:X\to Y$ is bijective, the cardinality of $X$ and $Y$ are the same.
\end{theorem}
An easy corollary of \cref{thm:bigtheorem} is the following:
\begin{corollary}
If $f:X\to Y$ is bijective, 
the cardinality of $X$ is at least as large as that of $Y$.
\end{corollary}
\begin{assumption}
The set $X$ is finite.
\label{ass:xfinite}
\end{assumption}
\begin{remark}
According to some, it is only the finite case (cf. \cref{ass:xfinite}) that is interesting.
\end{remark}
%restatable

\subsection{Citations and References}

Please use APA reference format regardless of your formatter
or word processor. If you rely on the \LaTeX\/ bibliographic
facility, use \texttt{natbib.sty} and \texttt{icml2024.bst}
included in the style-file package to obtain this format.

Citations within the text should include the authors' last names and
year. If the authors' names are included in the sentence, place only
the year in parentheses, for example when referencing Arthur Samuel's
pioneering work \yrcite{Samuel59}. Otherwise place the entire
reference in parentheses with the authors and year separated by a
comma \cite{Samuel59}. List multiple references separated by
semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
construct only for citations with three or more authors or after
listing all authors to a publication in an earlier reference \cite{MachineLearningI}.

Authors should cite their own work in the third person
in the initial version of their paper submitted for blind review.
Please refer to \cref{author info} for detailed instructions on how to
cite your own papers.

Use an unnumbered first-level section heading for the references, and use a
hanging indent style, with the first line of the reference flush against the
left margin and subsequent lines indented by 10 points. The references at the
end of this document give examples for journal articles \cite{Samuel59},
conference publications \cite{langley00}, book chapters \cite{Newell81}, books
\cite{DudaHart2nd}, edited volumes \cite{MachineLearningI}, technical reports
\cite{mitchell80}, and dissertations \cite{kearns89}.

Alphabetize references by the surnames of the first authors, with
single author entries preceding multiple author entries. Order
references for the same authors by year of publication, with the
earliest first. Make sure that each reference includes all relevant
information (e.g., page numbers).

Please put some effort into making references complete, presentable, and
consistent, e.g. use the actual current name of authors.
If using bibtex, please protect capital letters of names and
abbreviations in titles, for example, use \{B\}ayesian or \{L\}ipschitz
in your .bib file.

\section*{Accessibility}
Authors are kindly asked to make their submissions as accessible as possible for everyone including people with disabilities and sensory or neurological differences.
Tips of how to achieve this and what to pay attention to will be provided on the conference website \url{http://icml.cc/}.

\section*{Software and Data}

If a paper is accepted, we strongly encourage the publication of software and data with the
camera-ready version of the paper whenever appropriate. This can be
done by including a URL in the camera-ready copy. However, \textbf{do not}
include URLs that reveal your institution or identity in your
submission for review. Instead, provide an anonymous URL or upload
the material as ``Supplementary Material'' into the OpenReview reviewing
system. Note that reviewers are not required to look at this material
when writing their review.

% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
usually should) include acknowledgements.  Such acknowledgements
should be placed at the end of the section, in an unnumbered section
that does not count towards the paper page limit. Typically, this will 
include thanks to reviewers who gave useful comments, to colleagues 
who contributed to the ideas, and to funding agencies and corporate 
sponsors that provided financial support.

\section*{Impact Statement}

Authors are \textbf{required} to include a statement of the potential 
broader impact of their work, including its ethical aspects and future 
societal consequences. This statement should be in an unnumbered 
section at the end of the paper (co-located with Acknowledgements -- 
the two may appear in either order, but both must be before References), 
and does not count toward the paper page limit. In many cases, where 
the ethical impacts and expected societal implications are those that 
are well established when advancing the field of Machine Learning, 
substantial discussion is not required, and a simple statement such 
as the following will suffice:

``This paper presents work whose goal is to advance the field of 
Machine Learning. There are many potential societal consequences 
of our work, none which we feel must be specifically highlighted here.''

The above statement can be used verbatim in such cases, but we 
encourage authors to think about whether there is content which does 
warrant further discussion, as this statement will be apparent if the 
paper is later flagged for ethics review.


% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite
\nocite{langley00}

\section{Alternative views}
We have demonstrated the empirical success of layerwise linear models and argued that amplifying dynamics offers a unified framework for understanding their effectiveness. However, we also acknowledge and appreciate the existence of alternative perspectives.

\paragraph{Rigorous approach in a general setup}
Intuitive understandings can be vague, difficult to verify, and potentially misleading. Similar behaviors across different models may stem from unrelated causes. While intuitions are useful for communicating with a broader audience, researchers should prioritize rigorous theorems in general setups to avoid these pitfalls.

\paragraph{Essential non-linearity}
DNNs lose expressiveness and performance without non-linearities \cite{}. Some non-linearities may invalidate the amplifying dynamics and layerwise linear models could be too simplistic an approximation \cite{kunin2024get}, not warranting further focus. 

\paragraph{Response to alternative views}
In physics, even as quantum field theory and general relativity surpass Newtonian dynamics in accuracy, the simplicity of Newtonian models remains valuable for education and accessibility. Intuitive models can engage a wider audience, including new students and less specialized researchers, accelerating scientific progress.


\begin{comment}
\section{Introduction}
 Physicists often build intuition about complex natural phenomena by abstracting away intricate details—for instance, modeling a cow as a sphere \cite{kaiser2014sacred}, linearizing pendulum motion \cite{huygens19661673}, or using simplified frameworks like Hopfield networks to explore associative memory and network dynamics \cite{hopfield2007hopfield}. These abstractions enable tractable analysis while preserving the core principles of the system. A good model not only allows analytical solutions but also captures the underlying principle, often providing insights and extending their utility beyond their formal limits.   
\ys{Mention LLMs and attention, cite architecutres and interesting stuff in the introduction.}

Neural network are complex dynamical systems, with non-linearities often seen as their defining feature, complicating abstraction. Yet, simple layerwise linear models provide analytic solutions that capture key DNN phenomena beyond their limits (e.g., \cite{baldi1989neural,saxe2013exact}, see \cref{app:background} for a detailed review), highlighting the importance of layerwise structure and calling for deeper principles to understand it.

%Neural network dynamics are similarly complex, with non-linearities hindering abstraction. While rigorous results for general setups are valuable, they often rely on intricate theorems that obscure intuition. Linear neural networks and their variants serve as good starting models. 

%In this paper, we addresses the following question: what is the simplest key idea that describe DNN dynamics?

%In this paper, we demonstrated how the amplifying dynamics principle, realized through layerwise linear models even without non-linearities, is a defining characteristic of DNNs. We advocate for more work on this direction, as previous works are already successful in explaining practical DNN phenomena far beyond the models' scope.

%We advocate for greater attention and further exploration in this direction given its success in explaining practical DNN phenomena far beyond the models' scope.
%"In this paper, we position the amplifying dynamics principle, realized through layerwise linear models even without non-linearities, as a defining characteristic of deep neural networks.

In this paper, we propose the amplifying dynamics of layerwise models under gradient descent, where the growth of one layer is proportional to that of others, as an intuitive unifying principle. From this priciple, we highlight the significance of existing solvable layerwise linear models and how we can intuitively explain key DNN phenomena such as staircase learning, emergence, Neural Collapse, selective layer learning, rich/lazy training, and grokking from layerwise structure, gradient descent, and initialization.




\subsection{Position}
%\textbf{We advocate for greater attention to and further research on models based on the amplifying dynamics principle (layerwise linear models).}
\textbf{Our position is twofold: we advocate a greater attention on the success of layerwise linear models in describing/explaining neural network phenomena. In light of this, we call for new studies on amplifying dynamics, the unifying principle behind their effectiveness.}\ys{For scientific approach toward DNNs, we call for new studies...}
\end{comment}


\section{Discussion}
We have demonstrated the empirical success of layerwise linear models and proposed that amplifying dynamics serve as a unified framework for understanding their effectiveness. Specifically, we have explored the insights these models provide into the dynamics of neural networks. Beyond this, such models have also been applied to understand various phenomena, including modularization \cite{jarvis2024specialization,zhangunderstanding}, specialization \cite{jarvis2024theory}, fine-tunning \cite{lipplinductive}, generalization \cite{advani2020high}, and neuroscience, as discussed in previous studies \cite{nelli2023neural,saxe2019mathematical,flesch2022orthogonal,farrell2023lazy,richards2019deep,lippl2024mathematical}. While our investigation has focused on two layer feed forward networks, it is important to highlight other architectures where linearization has been successfully employed to gain insights into their behavior, (eg.Deep networks \cite{}, CNN \cite{pinson2023linear}, RNN \cite{heij2007introduction}, Self supervised learning set up \cite{simon2023stepwise} and Transformers architecture \cite{ahn2023linear,katharopoulos2020transformers} ).

While these methods offer significant insights, we acknowledge their limitations and recognize the value of alternative perspectives that contribute to a more holistic understanding of neural networks.

%\paragraph{Rigorous approach in a general setup}
%Intuitive understandings can be vague, difficult to verify, and potentially misleading. Similar behaviors across different models may stem from unrelated causes. While intuitions are useful for communicating with a broader audience, researchers should prioritize rigorous theorems in general setups to avoid these pitfalls.

\subsection{Alternative view}

%\paragraph{Limited architecture}
%Practically successful DNNs are not simple 2-layer MLPs but complex architectures like convolutional neural networks or transformers, enhanced by normalizations and skip connections. We must incorporate these architectural innovations for understanding the success of DNNs.

\paragraph{Essential non-linearity}
DNNs lose expressiveness and performance without non-linearities. Some non-linearities may invalidate the amplifying dynamics and layerwise linear models could be too simplistic an approximation \cite{kunin2024get}, not warranting further focus. 

\paragraph{Response to Alternative Perspectives}
In physics, while quantum field theory and general relativity surpass Newtonian dynamics in accuracy, the simplicity of Newtonian models continues to hold significant value. These models aid in developing intuition, guiding our understanding, and advancing the types of problems we can solve. Furthermore, intuitive models are more accessible to a broader audience, fostering engagement and accelerating scientific progress.


\section{Conclusion}
In this paper, we demonstrated how the amplifying dynamics principle, realized through layerwise linear models, explains practical DNN phenomena far beyond their original scope. From this principle, sigmoidal dynamics and stage-like training explain emergence; greedy dynamics toward salient features predicts Neural Collapse; weight imbalances determine which layers are learned or fixed; and the ratio of initial to target norms clarifies grokking's overfitting phase. 

These insights highlight the layerwise structure, even without non-linearity, as a defining characteristic of DNNs. We propose amplifying dynamics as a cornerstone for a unified, simplified theory of neural networks, paving the way for future machine learning textbooks. Accordingly, we reaffirm our call for research exploring this direction.

\subsection{Call of actions: research directions}

\paragraph{Connection to generalization} We empirically observe from NC and grokking that generalization often correlates with greedy dynamics. However, the connection between the inductive bias in dynamics and the inductive bias in generalization requires further research. 

\paragraph{Is learning all layers always better?} While we can control initialization to focus feature learning on specific layers, this raises intriguing questions: If only a few layers are utilized, wouldn't the solution resemble that of a shallow network? What, then, is the role of depth? Should we aim to gradually learn features across many layers, and if so, why is this progression beneficial? {\color{blue} As initially explored in \cite{kunin2024get,saxe2013exact,saxe2019mathematical}.}

\paragraph{Can we incorporate non-linearity?} Physics often employs perturbative or approximate models that extend simple systems. Given that ReLU is partially linear, can we similarly incorporate non-linearity into current layerwise linear models to bridge the gap to more complex behaviors? 
{\color{blue} Several studies have laid the groundwork in this direction, highlighting the need for continued exploration \cite{kunin2024get,saxe2022neural,zhang2024bias}.}

\section{Proof Dump}
Then from \cref{eq:app:w2},
\begin{align}
\frac{dW_2}{dt}(I-V^TV) &= -W_1^T\mathbf{E}\left[xx^T\right]W_1W_2(I-V^TV) +W_1^T\mathbf{E}\left[xy^T\right](I-V^TV) \\
&= -W_1^T\mathbf{E}\left[xx^T\right]W_1W_2(I-V^TV)
\end{align}
where we used \cref{eq:app:eig_corr} in the second line and \cref{eq:app:epsilon} in the last line. Letting $P =I-V^TV$, the time evolution of the norm of $W_2P$ is
\begin{align}
\frac{d}{dt}||W_2P||_F &= \frac{d}{dt}Tr(PW_2^TW_2P)\\
&= -2Tr(PW_2^TW_1^T\mathbf{E}\left[xx^T\right]W_1W_2P) \\
&\leq 0.
\end{align}
where in the last line we used that $PW_2^TW_1^T\mathbf{E}\left[xx^T\right]W_1W_2P$ is positive semi-definite matrix.

Let $W_2(\infty) = RD_2V$ where $R \in \mathbb{R}^{p \times c}$ is a semi-orthogonal matrix where $R^TR = I_{c}$ with $I_{c}$ an identity matrix of rank $c$.


Then 
\begin{align}
(I_p-RR^T)W_1^TW_1(I_p-RR^T) - (I_p-RR^T)W_2W_2^T(I_p-RR^T) = \epsilon(I_P - RR^T)
\end{align}
and $\| W_1(I_p-RR^T) \|_F \leq \sqrt{\|\epsilon\|}$. Thus, any component of $W_1$ outside $c$ dimensions is bounded by $\epsilon$

\subsection{Solution for multiple 2-layer models}

{\bf (THIS WHOLE SECTION IS NOT USED YET, SO DON'T NEED TO EDIT)}

We consider the model of parallel(?) $2$-layers, with parameters $\vec{a}_i , \vec{b}_i \in \mathbb{R}^{n_i}$ ($i=1,2,\cdots, p$) to learn function of
\begin{equation}
f(x) = \frac{1}{Z}  (\vec{a}_1^t \vec{b}_1, \cdots, \vec{a}_p^t \vec{b}_p) \cdot (x_1, \cdots, x_p), \quad f^{*}(x) = S x_1
\end{equation}
and our dataset $X \in \mathbb{R}^{n \times p}$ consists of $n<p$ datasets of length $p$ vectors. We denote our loss as
\begin{equation}
\mathcal{L}_X =  \frac{1}{2} | X (\vec{v}_f - \vec{v}_{f^{*}} )|^2, \quad \vec{v}_f = Z^{-1} (\vec{a}_1^t \vec{b}_1, \cdots, \vec{a}_p^t \vec{b}_p), \quad \vec{v}_{f^*} = (S,0,\cdots, 0).
\end{equation}
Write $Q : \mathbb{R}^p \rightarrow \mathbb{R}$ as $Q(\vec{w}) = \frac{1}{2} \| X \vec{w} \|^2$. We note that
\begin{equation}
Q_i(\vec{w}) = \frac{\partial Q}{\partial w_i}(w_1, \cdots, w_p) = \vec{e}_i^t X^t X \vec{w}, \quad \nabla_{\vec{w}} Q = (Q_1(\vec{w}), \cdots, Q_p(\vec{w})) = X^t X \vec{w}.
\end{equation}
Our gradient descent dynamics for $\vec{a}_i, \vec{b}_i$ are given as
\begin{align}
\frac{d}{dt} \vec{a}_i &= \nabla_{\vec{a}_i} \mathcal{L}_X = -\nabla_{\vec{a}_i}  Q(Z^{-1} \vec{a}_1^t \vec{b}_1 - S, Z^{-1} \vec{a}_2^t \vec{b}_2, \cdots, Z^{-1} \vec{a}_p^t \vec{b}_p ) \\
&= - Q_i (\vec{v}_f - \vec{v}_{f^*}) \cdot \nabla_{\vec{a}_i} (Z^{-1} \vec{a}_i^t \vec{b}_i) \\
&= - Z^{-1} Q_i (\vec{v}_f - \vec{v}_{f^*} ) \vec{b}_i
\end{align}
and similarly
\begin{equation}
\frac{d}{dt} \vec{b}_i = - Z^{-1} Q_i(\vec{v}_f - \vec{v}_{f^{*}} ) \vec{a}_i.    
\end{equation}
Write $Q_i$ simply as $Q_i(\vec{v}_f - \vec{v}_{f^*})$, unless stated otherwise. We have
\begin{equation}
\frac{d}{dt} (\vec{a}_i + \vec{b}_i) = - Z^{-1} (\vec{a}_i + \vec{b}_i) Q_i, \quad \frac{d}{dt} (\vec{a}_i - \vec{b}_i ) = Z^{-1} (\vec{a}_i - \vec{b}_i) Q_i
\end{equation}
so if we define
\begin{equation}
\gamma_i (t) = \exp \left(- 2 \int_{0}^{t} Z^{-1} \left( Q_i|_{t=s} \right) ds \right)
\end{equation}
then we have
\begin{equation}
\vec{a}_i(t) + \vec{b}_i(t) = \gamma_i(t)^{1/2}(\vec{a}_i(0) + \vec{b}_i(0)), \quad  \vec{a}_i(t) - \vec{b}_i(t) = \gamma_i(t)^{-1/2} (\vec{a}_i(0) - \vec{b}_i(0) )
\end{equation}
and $\gamma_i$ satisfies the dynamics of
\begin{equation}
\gamma_i(0) = 0, \quad \frac{d\gamma_i}{dt} = - 2 Z^{-1} \gamma_i Q_i.
\end{equation}
We can express $\vec{a}_i^t \vec{b}_i$ using $\gamma_i$ as
\begin{equation}
    \vec{a}_i^t \vec{b}_i = \frac{|\vec{a}_i + \vec{b}_i|^2}{4}  - \frac{|\vec{a}_i - \vec{b}_i|^2}{4} = s_i^{+} \gamma_i - s_{i}^{-} \gamma_i^{-1}, \quad s_{i}^{\pm} = \frac{|\vec{a}_i(0) \pm \vec{b}_i(0)|^2}{4}
\end{equation}
and express the entire dynamics in $\gamma_i$. Meanwhile, we can observe
\begin{equation}
    \frac{d}{dt} (\log \gamma_1, \cdots, \log \gamma_p)  = - (Q_1, \cdots, Q_p) =  \nabla_{\vec{w}} Q(\vec{v}_f - \vec{v}_{f^{*}}) \in \mathrm{im}(X^t)
\end{equation}
and as $\log \gamma_i(0)=0$, it follows that the dynamics of $\vec{v}_f$ always stay in the region
\begin{equation}
\vec{v}_f  \in \mathcal{D}(\mathrm{im}(X^t) , (s_i^{\pm})_i ) = \{ (s_1^{+} \gamma_1 - s_1^{-} \gamma_1^{-1} , \cdots, s_p^{+} \gamma_p - s_p^{-} \gamma_p^{-1} ) \, | \, \gamma_i >0,  (\log \gamma_1, \cdots, \log \gamma_p) \in \mathrm{im}(X^t) \}.
\end{equation}

\begin{theorem}
Suppose that $s_i^{\pm} \neq 0$ for all $i$, and $\vec{v}$ be any vector, $V$ be any subspace of dimension $p$. Then the submanifold $\mathcal{D}(V ,(s_i^{\pm})_i) \subset \mathbb{R}^p$ intersects with $V^{\perp} + \vec{v}$ at a single point $\mathfrak{p}\left(V; (s_i^{\pm})_i, \vec{v} \right)$, and the intersection is transversal. Furthermore, the gradient descent dynamics converges $\vec{v}_f \rightarrow \mathfrak{p}\left(\mathrm{im}(X^t); (s_i^{\pm})_i, \vec{v} \right)$.
\end{theorem}

\begin{proof}
(to be filled... let me revisit it later. boundness of dynamics - accumulation point exists - that point should be converging - existence - calculate derivative to show intersection is transversal - unique by showing no two such points exist)
\end{proof}

We want to consider the limit of this intersection point when initial condition goes to zero. We show that the 'limit' of the dynamics region $\mathcal{D}(\mathrm{im}(X^t) ,s_i^{\pm})$ exists if $s_i^{+}, s_i^{-}$ converge to zero satisfying certain conditions. We will describe the region $\mathcal{D}_{\infty}(V)$ first before we describe our theorem. For a partition
\begin{equation}
\{1,\cdots, p\} = I_{+}\sqcup I_{-} \sqcup I_{0}, \quad |I_0| = p-n
\end{equation}
define the set
\begin{equation}
\mathcal{B}(I_{+},I_{-},I_{0} ) = \{ (x_1, \cdots, x_p) \in [-1,1]^p : x_i = 1 \text{ if } i \in I_{+}, \, x_i = -1 \text{ if } i \in I_{-} \}
\end{equation}
and
\begin{equation}
    \mathcal{Q} (I_{+}, I_{-}, I_{0}) = \{ (x_1, \cdots, x_p)  \in \mathbb{R}^p : x_i \ge 0 \text{ if } i \in I_{+}, \, x_i \le 0 \text{ if } i \in I_{-}, \, x_i = 0 \text{ if } i \in I_{0} \} .
\end{equation}
Our set $\mathcal{D}_{\infty}(V)$ is described as
\begin{equation}
    \mathcal{D}_{\infty}(V) = \bigcup_{\mathcal{B}(I_{+},I_{-}, I_{0}) \cap V \neq \emptyset } \mathcal{Q}(I_{+},I_{-},I_{0} ).
\end{equation}

Define the genericity condition (GC) on $V$ as : $V$ does not contain a vector such that $(n+1)$ of its entries are either $1$ or $-1$, and it intersects transversally with all $(p-n)$-dimensional coordinate hyperplanes. (trying to figure out how to describe this well)

\begin{theorem}
Let $V$ be a $n$-dimensional subspace such that $V$ does not contain a vector such that $(n+1)$ of its entries are either $1$ or $-1$, and it intersects transversally with all $(p-n)$-dimensional coordinate hyperplanes.
\begin{enumerate}
\item Suppose $\vec{u} \in \mathcal{D}_{\infty}(V)$. Then for any given $\epsilon>0$ and $\gamma>1$, there exists $M>0$ such that
\begin{equation}
B_{\epsilon}(\vec{u}) \cap \mathcal{D}\left(V,(s_i^{\pm})_i \right) \neq \emptyset
\end{equation}
for any $s_i^{\pm}$ satisfying $\min_i(s_i^{\pm}) > M$ and $\max_{i,j}(s_i^{\pm}/s_j^{\pm}) < \gamma$. ( $B_{\epsilon}(\vec{u}) = \{ \vec{x} : | \vec{u}  - \vec{x}| < \epsilon \}$)
\item Suppose $\vec{u} \notin \mathcal{D}_{\infty}(V)$. Then for any $\gamma>1$, there exists $M>0$ and $\epsilon>0$ such that
\begin{equation}
B_{\epsilon}(\vec{u}) \cap \mathcal{D}\left(V,(s_i^{\pm})_i \right) = \emptyset
\end{equation}
for any $s_i^{\pm}$ satisfying $\min_i(s_i^{\pm}) > M$ and $\max_{i,j}(s_i^{\pm}/s_j^{\pm}) < \gamma$.
\end{enumerate}
\end{theorem}

\begin{proof}
Write $\vec{u} = (u_1, \cdots, u_p)$. We can consider $\prod_{i=1}^{p} (u_i - \epsilon, u_i + \epsilon)$ instead of $B_{\epsilon}(\vec{u})$. \\

(to be filled)
\end{proof}

Now define
\begin{equation}
    \mathfrak{p}(V;\vec{v}) =  \mathcal{D}_{\infty}(V) \cap \left(V^{\perp} + \vec{v} \right).
\end{equation}

\begin{theorem}
Let $V$ be a $n$-dimensional subspace satisfying the condition of Theorem F.2. Then for any vector $\vec{v} \in \mathbb{R}^n \setminus 0$, $\mathcal{D}_{\infty}(V)$ intersects with $V^{\perp} + \vec{v}$ at one point transversally, and the intersection $\mathfrak{p}(V;\vec{v})$ satisfies
\begin{equation}
\lim_{\min(s_i^{\pm}) \rightarrow \infty, \max(s_i^{\pm}/s_j^{\pm})<\gamma } \mathfrak{p}(V;(s_i^{\pm})_i,\vec{v})  = \mathfrak{p}(V;\vec{v})
\end{equation}
for any $\gamma>1$.
\end{theorem}

\begin{proof}
(combine Theorem F.1 and Theorem F.2, should be easy (but annoying) exercise)
\end{proof}

We finally discuss the distribution of $\mathfrak{p}(V;\vec{v})$ when $V$ follows unique isotropic distribution in all dimension $n$ subspaces of $\mathbb{R}^p$ (uniform distribution in orthogonal Grassmannian $\mathrm{Gr}(n,p)$ to put exactly).


\begin{theorem}
For $\vec{v}_{f^{*}} = (S,0, \cdots, 0)$, denote
\begin{equation}
f(n,p) = P_{V \sim \text{uniform}(\mathrm{Gr}(n,p))} \left( \mathfrak{p}(V; \vec{v}_{f^*} ) = \vec{v}_{f^{*}} \right).
\end{equation}
Then it satisfies:
\begin{enumerate}
\item $f(1,p) = \frac{1}{p}.$
\item $n_1<n_2 \Rightarrow f(n_1,p) < f(n_2,p)$.
\item $(1-f(n_1 + n_2,p)) \le (1-f(n_1,p)) (1-f(n_2,p))$. In particular, $f(n,p) \ge 1 - (1-\frac{1}{p})^n$.
\end{enumerate}
\end{theorem}

\begin{proof}
We first show that $\mathfrak{p}(V;\vec{v}_{f^*} ) = \vec{v}_{f^*}$ if and only if $V$ intersects with the affine cone
\begin{equation}
C = \{(x_1, \cdots, x_p) \in \mathbb{R}^ p : |x_1| = \max(|x_1|, \cdots, |x_p| ) \}.
\end{equation}
(need to fill details)
\end{proof}
It seems that there is no easy formula for $f(n,p)$, as you can see from the example
\[
f(2,3) = \frac{2}{\pi} \sin^{-1}   \left(\frac{1 }{3} \right) \approx 0.216347.
\]

Generally we can show that
\[
f(p-1,p) = P_{Y_1, \cdots, Y_p \sim N(0,1) \text{ iid}}\left(|Y_1| < |Y_2|+ \cdots + |Y_p| \right)
\]
\begin{proof}
Let $(y_1, \cdots, y_p)$ be orthogonal complement of $(p-1)$-dimensional subspace $V$. If $|y_1|>|y_2| + \cdots + |y_p|$, then $\vec{0} \neq (x_1, \cdots, x_p) \in V$ implies \begin{equation}
    |x_1| = \frac{|-y_2 x_2 - \cdots - y_p x_p|}{|y_1|} \le \frac{|y_2| + \cdots + |y_p|}{|y_1|} \max (|x_2|, \cdots, |x_p|) < \max (|x_2|, \cdots, |x_p|)
\end{equation}
so $V$ does not intersect with $C$ except at $0$. If $|y_1| \le |y_2| + \cdots + |y_p|$ then one can check
\begin{equation}
\left(\frac{|y_2| + \cdots + |y_p|}{|y_1|}, -\mathrm{sgn}(y_2), \cdots, -\mathrm{sgn}(y_p)\right) \in V  \cap C.
\end{equation}
Observe that choosing $V$ in uniform measure is equivalent to choosing $(y_1, \cdots, y_p)$ following the isotropic normal distribution $N(\vec{0}, I_p)$.
\end{proof}
As $E[|Y|] = \sqrt{\frac{2}{\pi}}$ and $V[|Y|] = 1 - \frac{2}{\pi}$, for $W = |Y_2|  + \cdots + |Y_p| - |Y_1|$ we have $\mathbb{E}[W] = (p-2) \sqrt{\frac{2}{\pi}}$ and $V[W] = p \left( 1 - \frac{2}{\pi} \right)$. Naive approximation using CLT (for large $p$) gives
\begin{equation}    
1 - f(p-1,p) = P(W<0) \approx  \frac{1}{2} \mathrm{erfc} \left( \frac{\mathbb{E}[W]}{\sqrt{2V[W]}} \right) \approx \sqrt{\frac{\pi-2}{4 \pi}}p^{-1/2} 
e^{-\frac{1}{\pi-2} p}
\end{equation}
where we have used $\mathrm{erfc}(z)  \approx \pi^{-1/2} z^{-1} e^{-z^2}$.

When $n=1$, distribution of $\mathfrak{p}(V;\vec{v}_{f^*})$ can be described rather concretely.

Choosing $V$ uniformly among $1$-dimensional subspace is equivalent to choosing $(X_1, \cdots, X_p) \sim N(\vec{0}_p, I_p)$ as isotropic normal and set $V = \mathrm{span}((X_1, \cdots, X_p) )$. Then $\mathcal{D}_{\infty}(V)$ becomes $\mathrm{span}(\vec{e}_i) $ for $i = \mathrm{argmax}_j ( |X_j| )$. Its intersection with $V^{\perp} + \vec{v}_{f^{*}}$ is given as
\begin{equation}
\mathfrak{p}(V;\vec{v}_{f^*}) = S\frac{X_1}{X_i} \vec{e}_i, \quad i = \mathrm{argmax}_{j}\left( |X_j| \right).
\end{equation}

\subsection{Derivation of orth-direction}
For sufficiently small initialization, any matrix is sufficiently similar to the assumed form.  and 
we show that $\alpha_i = u_i^TW_1W_2v_i$ maps to a decoupled mode of the dynamics.

\cref{eq:app:epsilon} dictactes that we can From the derivation above and assuming $W_1^TW_1=W_2W_2^T$, we can assume $W_1 = U^TAR$ and $W_2=R^TAV$ where $R \in \mathbb{R}^{c \times c}$  is an orthogonal matrix and $A$ are diagonal matrices. Then 

\begin{align}
u_i^T\frac{dW_1}{dt}W_2v_i &= -u_i^T\mathbf{E}\left[xx^T\right]W_1W_2W_2^TW_2v_i\ +u_i^T\mathbf{E}\left[xy^T\right]W_2^TW_2v_i \\
u_i^TW_1\frac{dW_2}{dt}v_i &= -u_i^TW_1W_1^T\mathbf{E}\left[xx^T\right]W_1W_2v_i\ +u_i^TW_1W_1^T\mathbf{E}\left[xy^T\right]v_i \\
\end{align}

\begin{align}
u_i^T\frac{dW_1}{dt}W_2v_i &= -a_i^4\ +\rho_ia_i^2 \\
u_i^TW_1\frac{dW_2}{dt}v_i &= -a_i^4\ +\rho_ia_i^2\\
\end{align}








Because $W_1(\infty)W_2(\infty)x=y$ for all $(x,y)$, 
Because $W_1^TP\mathbf{E}\left[xx^T\right]W_1$ is positive semi-definite matrix, the norm of 


Then we from \cref{eq:app:w1},
\begin{align}
(I-UU^T)\frac{dW_1}{dt} &= -(I-UU^T)\mathbf{E}\left[xx^TW_1W_2W_2^T\right] +(I-UU^T)\mathbf{E}\left[xy^T\right]W_2^T \\
&= -(I-UU^T)\mathbf{E}\left[xx^T\right]W_1W_2W_2^T \\
&=
-(I-UU^T)\mathbf{E}\left[xx^T\right]W_1W_1^TW_1 + (I-UU^T)\mathbf{E}\left[xx^T\right]W_1\epsilon.
\end{align}
where we used \cref{eq:app:eig_corr} in the second line and \cref{eq:app:epsilon} in the last line. Letting $P =I-UU^T$, the time evolution of the norm of $PW_1$ is
\begin{align}
\frac{d}{dt}||PW_1||_F &= \frac{d}{dt}Tr(PW_1W_1^TP)\\ 
&= -2Tr(P\mathbf{E}\left[xx^T\right]W_1W_1^TW_1W_1^TP + P\mathbf{E}\left[xx^T\right]W_1\epsilon W_1^TP) \\
&=-2Tr(PW_1W_1^TW_1W_1^TP) \\
&\leq 0,
\end{align}
where in the last line we used $\mathbf{E}[xx^T]= I$ and took $\epsilon \rightarrow 0$.
Because $W_1^TP\mathbf{E}\left[xx^T\right]W_1$ is positive semi-definite matrix, the norm of 

The multitask sparse parity problem

They showed that quanta model with emergent property can reproduces the scaling laws observed in a 2-layer MLP trained on the multitask sparse parity problem.
in which the task was composed of discrete subtasks that follow a power-law. They also assumed that these quantazied subtasks (skills) were learned abruptly depending whether a criteria is met or not. Using the quanta model with power-law dataset, they were able to explain scaling law with emergence (Sudden gain). As a specific example of the model, they proposed the multitask sparse parity problem.


The objective of multitask sparse parity problem is to read the control and skills bits and calculate the parity function of the relevant bits. The position of the relevant bits - colored in the Skill bits column - differ among the skills, and the challenge lies in understanding that control bits indicate a skill and figuring out the relevant bits in the skill bits.
    
    In the sparse parity problem, .. skill bits are presented to the model. The target function is a parity function applied to a fixed subset of the input bits. The model must detect the relevant $m < \nb$ sparse bits and return the parity function on this subset ($M(i,x)$, see \cref{tab:multitask}). Michaud et al. \cite{michaud2023quantization} introduced the \textbf{multitask} sparse parity problem by introducing ?? unique sparse parity variants -- or skills -- with different sparse bits (for a representation, see \cref{tab:multitask}). 
Each skill is represented in the ?? control bits as a one-hot string, and the model must solve the specific sparse parity task indicated by the control bits 
    
     
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\columnwidth]{icml2024/figures/skill_table (cropped) (pdfresizer.com).pdf}%
    \vspace{-0.3cm}
    \caption{\textbf{Multitask sparse parity task} Table 1 from Nam et al.~\citeyear{nam2024exactly}. }
\end{figure}

\paragraph{Multitask sparse parity problem.} (for more details, see \cref{app:multitask}).

\subsection{Multitask sparse parity}
\label{app:multitask}
The sparse parity task can be stated as follows: for a bit string of length $n_b$, the goal is to determine the parity (sum mod 2) of a predetermined subset of $m$ bits within that string.  The \textbf{multitask} sparse parity \cite{michaud2023quantization} extends this problem by introducing  $\ns$  unique sparse parity variants in the dataset. The input bit strings have a length of $\ns + n_b$. The first $\ns$ bits function as indicators by assigning a specific task. The frequency of the distinct parity tasks follows a rank-frequency distribution with an inverse power law relation (power-law distribution).  The last $n_b$ bits are uniformly distributed. This sets a binary classification problem  $\{0,1\}^{\ns + n_b} \rightarrow \{0,1\}$ where only a single bit of the initial $\ns$ bits is nonzero.
In \cref{tab:multitask_app}, the many distinct parity tasks represent different skills.\,\footnote{Note that here we follow the even/odd parity convention used in \cite{michaud2023quantization}, i.e., $\{0,1\}$, instead of $\{1, -1\}$ as used in the main text.}


Representation of the multitask sparse parity as presented in \cite{michaud2023quantization}. The control bits are one-hot vectors encoding a specific parity task. The frequency of the different tasks follows a power-law distribution. In this example, there are $n_s =10$ tasks, and skill bits are length $n_b =15$. The $y$ column is the resulting parity computed from $m=3$ bits (highlighted in colors).  The multitask dataset provides a controlled experimental setting designed to investigate skills. 

The proposal in \cite{michaud2023quantization} aims to reconcile the regularity of scaling laws with the emergence of abilities with scale using three key hypotheses: (i) skills, represented as a
finite set of computations, are distinct and separate; (ii) these skills differ in their effectiveness,
leading to a ranking based on their utility to reduce the loss; and (iii) the pattern of how
frequently these skills are used in prediction follows a power-law distribution.  Interestingly,  the multitask problem has a consistent pattern across scaling curves: each parity displays a distinct transition, characterized by a sharp decrease in loss at a specific scale of parameters, data, or training step. Such a sudden shift occurs after an initial phase of no noticeable improvement, leading to reverse sigmoid-shaped learning curves. 
Michaud et al. \cite{michaud2023quantization} empirically show that for a one-hidden-layer neural network with ReLU activation, trained using cross-entropy loss and the Adam optimizer, these transitions happen at different scales for distinct tasks. This results in a smooth decrease in the overall loss as the number of skill levels increases.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.55\textwidth]{icml2024/figures/NC.drawio.pdf}%
    \includegraphics[width=0.45\textwidth]{icml2024/figures/pdfresizer.com pdf-crop.pdf}%
    \vspace{-0.3cm}
    \caption{\textbf{Illustration of Neural Collapse and Unconstrained feature model} \textbf{(a):} At the terminal stage of training, last layer features vectors (the post-activation of the penultimate layer), illustrated as colored dots, cluster by their class mean vector, illustrated as colored arrow and form a simplex ETF structure (orthogonal vectors projected at the compliment of the global mean vector). \textbf{(b):} The original unconstrained feature model (UFM) trains two matrices $H$ (representing the feature matrix) and $W_2$ (the last layer weights). We assumed a realizable condition and replaced the $H$ with $XW_1$ where $X$ represents the input features of the training set and $W_1$ first layer. The NC can be interpreted as the collapse of the rank of the feature matrix into $c$(number of classes) while $n$ (number of datapoints) and $p$ (the width of the last layer) are larger than $c$.\ys{clean me! Emphasize why NC is interesting}}\label{fig:app:NC}
\end{figure}

\section{Explicit solution for the 2-layer linear neural network with scalar input and scalar output}\label{app:lee}

We provide a general solution for the $2$-layer layerwise model described in \cref{eq:one_linear_nn}. To repeat the setting, our model and target functions are single variable functions  
\begin{equation}
f(x) = \frac{1}{Z}\left(  \sum_{i=1}^{p} a_i b_i  \right) x, \quad f^*(x) = Sx,
\end{equation}
where we can set our loss function as
\begin{equation} \label{eq:one_linear_nn_loss}
    \mathcal{L} = \frac{1}{2} \left( \frac{1}{Z} \sum_{i=1}^{p} a_i b_i - S \right)^2.
\end{equation}

\begin{theorem}
The solution for the gradient descent dynamics for the loss function (\cref{eq:one_linear_nn_loss}) is given as
\begin{align} \label{eq:one_linear_nn_sol_ab}
a_i(t) &= \frac{a_i(0) + b_i(0)}{2} \gamma(t)^{1/2} + \frac{a_i(0) - b_i(0)}{2} \gamma(t)^{-1/2}, \\
b_i(t) &= \frac{a_i(0) + b_i(0)}{2} \gamma(t)^{1/2} - \frac{a_i(0) - b_i(0)}{2} \gamma(t)^{-1/2},
\end{align}
where
\begin{equation}
    \gamma(t) = \frac{\Sigma_0 - \mathcal{S}_0 +S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}+\left(-\Sigma_0 + \mathcal{S}_0 -S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}\right)e^{-4 Z^{-1} \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2} t} }{
    \Sigma_0 + \mathcal{S}_0 -S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}+\left(-\Sigma_0 -\mathcal{S}_0 +S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}\right)e^{-4 Z^{-1} \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2} t}}
\end{equation}
and
\begin{equation}
\mathcal{S}_0 = \frac{1}{Z} \sum_{j=1}^{p} a_j(0) b_j(0), \quad \Sigma_0 = \frac{1}{Z} \sum_{j=1}^{p} \frac{a_j(0)^2+b_j(0)^2}{2}.\end{equation}
In particular, we have
\begin{equation}
    \lim_{t \rightarrow \infty} \gamma(t) = \gamma(\infty) = \frac{S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}}{\Sigma_0 + \mathcal{S}_0}.
\end{equation}
The function $\gamma$ is always monotone from $\gamma(0)=1$ to $\gamma(\infty)$: if $S> \mathcal{S}_0$ then $\gamma$ is increasing, and if $S<\mathcal{S}_0$ then $\gamma$ is decreasing.
\end{theorem}

\begin{proof}
Since our gradient descent dynamics is given as
\begin{align}
    \frac{d a_i}{dt} = -\frac{\partial \mathcal{L}}{\partial a_i} = - b_i \left( Z^{-2} \sum_{j=1}^{m}a_j b_j - Z^{-1} S \right), \quad  
    \frac{d b_i}{dt} = -\frac{\partial \mathcal{L}}{\partial b_i} = - a_i \left( Z^{-2} \sum_{j=1}^{m} a_j b_j - Z^{-1} S \right),
\end{align}
one can observe
\begin{align}
    \frac{d}{dt} (a_i + b_i) = -(a_i + b_i)\left( Z^{-2} \sum_{j=1}^{p}a_j b_j - Z^{-1}S \right), \quad  
    \frac{d}{dt} (a_i - b_i) = (a_i - b_i)Z^{-1} \left( Z^{-2} \sum_{j=1}^{p}a_j b_j - Z^{-1}S \right).
\end{align}

So if we define $\gamma$ as 
\begin{equation}
    \gamma(t) = \exp \left( -2 \int_{s=0}^{t} 
    \left( Z^{-2} \sum_{j=1}^{p}a_j(s) b_j(s) - Z^{-1} S \right) ds \right),
\end{equation}
then we have 
\begin{equation}
    \frac{d}{dt} \left( \gamma \right) = \gamma \left( -2  
     Z^{-2} \sum_{j=1}^{p}a_jb_j - Z^{-1} S \right).
\end{equation}
Hence 
\begin{align}
    \frac{d}{dt} \left( \gamma^{-1/2} (a_i + b_i) \right) &= \gamma^{-1/2}    \left( Z^{-2} \sum_{j=1}^{p}a_j b_j - Z^{-1} S \right) (a_i + b_i) - \gamma^{1/2}\left( Z^{-2} \sum_{j=1}^{p}a_j b_j - Z^{-1} S \right) (a_i + b_i) = 0, \\
    \frac{d}{dt} \left( \gamma^{-1/2} (a_i - b_i) \right) &= -\gamma^{-1/2}    \left( Z^{-2} \sum_{j=1}^{p}a_j b_j - Z^{-1} S \right) (a_i - b_i) + \gamma^{-1/2}\left( Z^{-2} \sum_{j=1}^{p}a_j b_j - Z^{-1} S \right) (a_i - b_i) = 0.
\end{align}
From those and $\gamma(0)=0$ we have
\begin{equation}
    a_i(t) + b_i(t) = (\gamma(t))^{1/2} (a_i(0) + b_i(0)), \quad a_i(t) - b_i(t) = (\gamma(t))^{-1/2} (a_i(0)-b_i(0) ),
\end{equation}
which leads to \cref{eq:one_linear_nn_sol_ab}. We next work on dynamics of $\gamma$. We start from
\begin{equation}
    \frac{1}{\gamma} \frac{d \gamma}{dt} = \frac{d}{dt}(\log \gamma) = -2 Z^{-2} \sum_{j=1}^{m} a_j b_j + 2Z^{-1} S.
\end{equation}
We can express
\begin{align}
    Z^{-2} \sum_{j=1}^{p} a_j b_j &=  Z^{-2} \sum_{j=1}^{p} \left( \frac{(a_j+b_j)^2}{4}  - \frac{(a_j - b_j)^2}{4} \right)\\ &= Z^{-2} \sum_{j=1}^{p} \frac{(a_j(0)+b_j(0))^2}{4} \gamma - Z^{-2} \sum_{j=1}^{p} \frac{(a_j(0)+b_j(0))^2}{4} \gamma^{-1} \\
    &= Z^{-2} \sum_{j=1}^{p} a_j(0) b_j(0) \frac{\gamma + \gamma^{-1}}{2} + Z^{-2} \sum_{j=1}^{p} \frac{a_j(0)^2+b_j(0)^2}{2} \frac{\gamma - \gamma^{-1}}{2}.
\end{align}
So if we denote
\begin{equation}
\mathcal{S}_0 = \frac{1}{Z} \sum_{j=1}^{p} a_j(0) b_j(0), \quad \Sigma_0 = \frac{1}{Z} \sum_{j=1}^{p} \frac{a_j(0)^2+b_j(0)^2}{2},
\end{equation}
then our dynamics for $\gamma$ becomes
\begin{equation}
\frac{d \gamma}{dt} = -2Z^{-1} \gamma \left(
\mathcal{S}_0 \frac{\gamma-\gamma^{-1}}{2} + \Sigma_0 \frac{\gamma + \gamma^{-1}}{2}- S\right) = -2 Z^{-1}\left( (\Sigma_0 + \mathcal{S}_0)\gamma^2 - 2 S \gamma - (\Sigma_0 - \mathcal{S}_0) \right).
\end{equation}
One can observe
\begin{equation}
\Sigma_0 = \frac{1}{Z} \sum_{j=1}^{p} \frac{a_j(0)^2+b_j(0)^2}{2} \ge \frac{1}{Z} \sum_{j=1}^{p} |a_j(0) b_j(0)| \ge |\mathcal{S}_0|,
\end{equation}
so we can always factor the quadratic in $\gamma$ as
\begin{equation}
(\Sigma_0 + \mathcal{S}_0)\gamma^2 - 2 S \gamma - (\Sigma_0 - \mathcal{S}_0) = (\Sigma_0 + \mathcal{S}_0) (\gamma - \gamma_{-})(\gamma- \gamma_{+})
\end{equation}
where
\begin{equation}
    (\gamma_{-}, \gamma_{+}) = \left( \frac{S - \sqrt{ \Sigma_0^2 -  \mathcal{S}_0^2 + S^2}}{ \Sigma_0 + \mathcal{S}_0}, \frac{S + \sqrt{ \Sigma_0^2 -  \mathcal{S}_0^2 + S^2}}{\Sigma_0 + \mathcal{S}_0} \right) \quad \Rightarrow \quad \gamma_{-}<0<\gamma_{+}.
\end{equation}
We continue using partial fraction decomposition as
\begin{equation}
\frac{1}{(\gamma- \gamma_{-}) (\gamma - \gamma_{+})} \frac{d \gamma}{dt} = \frac{1}{\gamma_{+} - \gamma_{-}}\left( \frac{1}{\gamma - \gamma_{+}}-\frac{1}{\gamma-\gamma_{-}} \right) \frac{d \gamma}{dt} = -2 Z^{-1} (\Sigma_0 + \mathcal{S}_0)
\end{equation}
and
\begin{equation}
\frac{d}{dt} \log \left| \frac{\gamma - \gamma_{+}}{\gamma - \gamma_{-}}  \right| = -2 Z^{-1} (\Sigma_0 + \mathcal{S}_0)(\gamma_{+} - \gamma_{-} ) = - 4Z^{-1} \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}.
\end{equation}
Both $\gamma - \gamma_{+}$ and $\gamma - \gamma_{-}$ do not change signs, so the following holds regardless of the sign of $\gamma- \gamma_{+}$:
\begin{equation}\label{eq:eqn75}
\frac{\gamma - \gamma_{+}}{\gamma- \gamma_{-}} = \frac{\gamma(0) - \gamma_{+}}{\gamma(0)-\gamma_{-}} \exp \left(-4Z^{-1} \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2} t \right)
\end{equation}
As $\gamma(0)=1$, this is solved as
\begin{equation}
    \gamma = \frac{\Sigma_0 - \mathcal{S}_0 +S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}+\left(-\Sigma_0 + \mathcal{S}_0 -S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}\right)e^{-4 Z^{-1} \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2} t} }{
    \Sigma_0 + \mathcal{S}_0 -S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}+\left(-\Sigma_0 -\mathcal{S}_0 +S + \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2}\right)e^{-4 Z^{-1} \sqrt{\Sigma_0^2 - \mathcal{S}_0^2 + S^2} t}}.
\end{equation}
Considering the limit of $t \rightarrow \infty$ at \cref{eq:eqn75} gives
\begin{equation}
    \gamma(t) \xrightarrow{t \rightarrow \infty} \gamma_{+} = \frac{S + \sqrt{ \Sigma_0^2 -  \mathcal{S}_0^2 + S^2}}{\Sigma_0 + \mathcal{S}_0}.
\end{equation}
From \cref{eq:eqn75} we can also see $\gamma \in (\gamma_{-}, \gamma_{+})$, and $\gamma$ increases if and only if $1 - \gamma_{+}>0$. It is straightforward to check that if $S>\mathcal{S}_0$ (or $S<\mathcal{S}_0$) then $\gamma_{+}>1$ (and $\gamma_{+}<1$ respectively).
\end{proof}

\begin{remark}
If $S>\mathcal{S}_0$, then the graph of $\gamma(t)$ becomes part of some sigmoid function whose image is $(\gamma_{-}, \gamma_{+})$ and center is at height $\frac{\gamma_{-} + \gamma_{+}}{2} = \frac{S}{\Delta_0+\Sigma_0}$. As the graph of $\gamma$ starts from height $1 = 
\gamma(0)$, one can show that $\gamma(t)$ is concave for all $t \ge 0$ if and only if $S<\Delta_0+\Sigma_0$, and otherwise it contains an inflection point. If $S< \mathcal{S}_0$, the graph takes a shape of (dilation and translation of) $(1-e^{-t})^{-1}$, so after the point $\gamma(0)=1$ it is convex and monotone decreasing.    
\end{remark}

\subsection{Set up for transformer}

\begin{tabular}{ c c c c c c  }
Name & Sub figure & Weight init ratio & Target scale & Input scale & Dropout rate \\
\hline\hline 
Default & (a) & 1 & 20 & 1 & 0 \\
Weight downscaling & (b) & \textbf{0.1} & 20 & 1 & 0 \\
Target upscaling & (c) & 1 & \textbf{20} & 1 & 0 \\
Input downscaling & (d) & 1 & 20 & \textbf{0.01} & 0 \\
Dropout & (e) & 1 & 20 & 1 & \textbf{0.8} 
\end{tabular}


\paragraph{Code} The code used to train transformer on modular division task was based on the code from \url{https://github.com/teddykoker/grokking}. We removed normalization, replaced tanh to ReLU, and replaced cross entropy to MSE loss for better similarity with the layerwise linear models in the main text.

\begin{figure}[ht] 
    \centering
    \subfloat[Grokking]{%
        \includegraphics[width=0.5 \columnwidth]{figures/transformer_acc.png}%
        }%
    \hfill
    \subfloat[Smaller initialization]{%
        \includegraphics[width=0.5 \columnwidth]{figures/transformer_acc_small_init.png}%
        }%
    \subfloat[Weaker input signal]{%
        \includegraphics[width=0.5 \columnwidth]{figures/transformer_acc_small_signal.png}%
        }%
    \hfill
    \subfloat[More datapoints]{%
        \includegraphics[width=0.5 \columnwidth]{figures/transformer_acc_large_data2.png}%
        }%
    \subfloat[Dropout]{%
        \includegraphics[width=0.5 \columnwidth]{figures/transformer_acc_dropout.png}%
        }%
    \caption{\textbf{Methods that remove grokking in mod p problem} A 2-layer transformer is trained with Adam on MSE loss. (a) Default scenario (b) the initialization weights of the token embedding were downscaled by a factor of $100$. (c) The token embeddings were divided by a factor of $100$ to mimic a smaller input signal. (d) $80\%$ instead of $50\%$ of the data were used as the training set. (e) Dropout with probability $0.6$ was applied to the last layer. [If out of space, use only two figures (grokking and one example of greedy dynamics)] and send everything else to appendix}\label{fig:removing_grokking_app}.  
\end{figure}


\begin{figure}[ht] 
    \centering
    \subfloat[Scaling initialization]{%
        \includegraphics[width=0.4 \columnwidth]{icml2024/figures/grokking/acc_init_wd0.0001_init_division.png}%
        }%
    \subfloat[Scaling embedding]{%
        \includegraphics[width=0.4 \columnwidth]{icml2024/figures/grokking/acc_init_wd0.0001_normalize_division.png}%
        }%
    \hfill
    \subfloat[Output scaling]{%
        \includegraphics[width=0.4 \columnwidth]{icml2024/figures/grokking/acc_init_wd0.0001_scaleOutput_division.png}%
        }%
    \subfloat[Width]{%
        \includegraphics[width=0.4 \columnwidth]{icml2024/figures/grokking/acc_init_wd0.0001_width_division.png}%
        }%
    \hfill
    \subfloat[Dropout]{%
        \includegraphics[width=0.4 \columnwidth]{icml2024/figures/grokking_grok_dropout_acc.pdf}%
        }%
    \subfloat[Output Downscaling]{%
        \includegraphics[width=0.4 \columnwidth]{icml2024/figures/grokking_grok_outshrink_acc.pdf}%
        }%
    \caption{\textbf{Grokking in MLP} ?????? }\label{fig:removing_grokking_app2_modular}.  
\end{figure}

\subsubsection{old version}
The assumption on $W_1$ and $W_2$ immediately shows that layers are balanced:
\begin{equation}\label{eq:app:epsilon}
W_1^TW_1 - W_2W_2^T = 0.
\end{equation}

Denote $u_i$ and $v_i$ be $i$th rows of $U$ and $V$ respectively. It follows that
\begin{align}
 W_1W_1^Tu_i = \alpha_i^2u_i, \quad W_2^TW_2v_i = \alpha_i^2v_i. 
\end{align}
Using \cref{eq:app:w1,eq:app:w2}, and we obtain the following equations:
\begin{align}
u_i^T\frac{dW_1}{dt}W_2v_i &= -u_i^T\mathbf{E}\left[xx^T\right]W_1W_2W_2^TW_2v_i\ +u_i^T\mathbf{E}\left[xy^T\right]W_2^TW_2v_i \\
u_i^TW_1\frac{dW_2}{dt}v_i &= -u_i^TW_1W_1^T\mathbf{E}\left[xx^T\right]W_1W_2v_i\ +u_i^TW_1W_1^T\mathbf{E}\left[xy^T\right]v_i 
\end{align}
By plugging in $\mathbf{E}[xx^T]=I$, $W_2^TW_2v_i = \alpha_i^2v_i$, $W_1W_1^Tu_i = \alpha_i^2u_i$, and $u_i^T\mathbf{E}\left[xy^T\right]v_i = \rho_i$, we obtain 
\begin{align}
u_i^T\frac{dW_1}{dt}W_2v_i &= -a_i^4\ +\rho_ia_i^2 \\
u_i^TW_1\frac{dW_2}{dt}v_i &= -a_i^4\ +\rho_ia_i^2.
\end{align}

Using the assumption, we get $u_i^TW_1W_2v_i = \alpha_i^2$. Then above equations become
\begin{align}
\frac{d\alpha_i^2}{dt} &= -2\alpha_i^2(\alpha_i^2- \rho_i^2) \quad \Rightarrow  \quad
\frac{\alpha_i^2(t)}{\rho_i} = \frac{1}{1+\left(\frac{\rho_i}{\alpha_i^2(0)} - 1\right)e^{-2 \rho_i t}}.
\end{align}

\paragraph{Discussion on the assumption} The assumption specifies a particular form for the matrix, but with sufficiently small initialization, all matrices approximately meet the conditions.
